Safe Reinforcement Learning with Model Uncertainty Estimates

Many current autonomous systems are being designed with a strong reliance on black box predictions from deep neural networks (DNNs). However, DNNs tend to be overconfident in predictions on unseen data and can give unpredictable results for far-from-distribution test data. The importance of predictions that are robust to this distributional shift is evident for safety-critical applications, such as collision avoidance around pedestrians. Measures of model uncertainty can be used to identify unseen data, but the state-of-the-art extraction methods such as Bayesian neural networks are mostly intractable to compute. This paper uses MC-Dropout and Bootstrapping to give computationally tractable and parallelizable uncertainty estimates. The methods are embedded in a Safe Reinforcement Learning framework to form uncertainty-aware navigation around pedestrians. The result is a collision avoidance policy that knows what it does not know and cautiously avoids pedestrians that exhibit unseen behavior. The policy is demonstrated in simulation to be more robust to novel observations and take safer actions than an uncertainty-unaware baseline.

==> background.tex <==
%!TEX root = main.tex

\section{Related Work} \label{sec:related_work}
This section investigates related work in safe reinforcement learning to develop a dynamic collision avoidance policy that is robust to out-of-data observations.

\subsection{Related Work}

\subsubsection{External novelty detection}
% Novelty detecter and safety controllers
Many related works use off-policy evaluation or external novelty detectors to verify the learner's returned policy (\cite{Richter_2017}, \cite{Long_2018}). These approaches place a threshold on the novelty detectors output and switch to a safety controller. This a) requires the knowledge of a safety controller that can act in a dynamic pedestrian environment or a high-speed traffic environment. B) there is no known possibility of gradually switching from an RL policy to a safety controller, because the safety controller has no knowledge about the RL's decision making process. A failure case would be a pedestrian in front of the vehicle, that is planned to be avoided by an action to the left of the RL and an action to the right of the safety controller. Our framework's trained knowledge of uncertainty maintains the capability of predicting observed pedestrians behaviors while gradually staying further away from unpredictable and uncertain regions. 

% Supervised learning approach from Richter is not possible
% Richter et al. avoids static obstacles via detecting novel images and switching to a safety controller \cite{Richter_2017}. However, his supervised approach is not scalable to dynamic collaborative agents and his work assumes a prior map to design useful safety controllers. In these kind of approaches a switch to safety controllers is possible in a binary way, as multiplying the output of, e.g. a reinforcement learner would undermine the decision authority and cause crashes in regions that have been predicted not to be safe. 
\subsubsection{Risk-sensitive RL}
% Explain two uncertainties
% Collisions can be pre-identified by high model uncertainty
This work focuses on detecting novel observations via model uncertainty, also known as parametric or epistemic uncertainty \cite{Kendall_2017}. This is orthogonal to and combinable with the field of risk-sensitive RL that focuses on environment uncertainty, also known as risk, inherent, or aleatoric uncertainty \cite{Gal_2016Thesis}. Environment uncertainty captures the uncertainty due to imperfect observations of the environment, e.g. inherent stochasticity, sensor noise, or the inability to observe the pedestrian's decision making process \cite{Gal_2016Thesis}. It cannot be explained away with data, but RL accounts for environment uncertainty, as it occurs during training, by incorporating it in the mean expected reward criterion~\cite{Tamar_2015}. Risk-sensitive RL which is often used in Online Learning extends the optimality criterion of the expected reward with measures of risk from financial literature such as \textit{Value-at-Risk} to be more sensitive to improbable events that have high cost \cite{Geibel_2006, Mihatsch_2002, Shen_2013, Tamar_2015, Evendar_2006}.
% TODO work over this the environment uncertainty here.

\subsubsection{Measures of model uncertainty}
Model uncertainty, in comparison, captures how well our model fits the possibilities of observations form the environment and could be explained away with infinite observations \cite{Gal_2016Thesis}. In applications with limited training data or test data that is far from the training data the model uncertainty is typically high \cite{Gal_2016Thesis}. Thus, it captures the moments in which our model fails to generalize to unseen test data and hints when we should not trust our network's predictions \cite{Gal_2016Thesis}.
% (SEE MIKE's collisions with high Uncertainty)

% Bayesian is expensive
Measures of model uncertainties in neural networks have recently gained significant attention. Most work uses Bayesian Neural Networks that measure model uncertainty by keeping track of a distribution of each weight instead of a single value \cite{MacKay_1992}. However, they require a significant restructuring of the network architecture and even approximate forms, such as Markov Chain Monte Carlo (MCMC) methods or variational inference, come with extensive computational cost and have a sample dependent accuracy \cite{Neal_1996}.

% Methods of approximate uncertainty with minimal architecture change
A newly emerging field finds approximations of Bayesian inference without significantly changing the neural network's architecture. Bootstrapping have been explored to generate approximate uncertainty measures to guide exploration \cite{Osband_2016}. By training a \textit{deep ensemble} of networks on partly overlapping dataset samples they agree in areas of common data and disagree, or have a sample variance, in regions of uncommon data \cite{Lakshmi_2016}. Dropout can be interpreted similarly, if activated during test-time, and has been shown to approximate Bayesian inference in Gaussian processes (\cite{Dropout_2014}, \cite{Gal_2015}). An alternative approach uses \textit{Hypernets}, a network that learns the weights of another network, to directly give parameter uncertainty values, but it showed computationally too expensive \cite{Pawlowski_2017}. A recent approach claims to retrieve bayesian uncertainty estimates via batch normalization, but remains with doubts in the analysis~\cite{Teye_2018}. Finally, we are leveraging Dropout and Deep Ensembles to guide our agent away from unknown pedestrian behavior. 
% TODO: bayes by backprop
%\cite{Lakshmi_2016} uses \textit{deep ensembles} and adversarial training to give predictive uncertainty estimates. 
% Gal and Ghahramani have proposed have proposed \textit{Monte Carlo Dropout} (MC-dropout) to approximate , which is traditionally used as regularization . (However, dropout tends to underestimate the uncertainty for out-of-distribution data).  

% We cannot use approaches from risk-affine / uncertainty-guided exploration
\subsubsection{Applications of model uncertainty in RL}
Measures of model uncertainty have been used in RL very recently to speed-up training by guiding the exploration into regions of high uncertainty \cite{Thompson_1933, Osband_2016, Liu_2017}. Kahn et al. has used model uncertainty estimates for static obstacle collision avoidance. This work extends his framework to the highly complex domain of pedestrian collision avoidance. It additionally identifies the major dilemma of that a uncertainty-averse policy is safe in execution, but won't explore during training, whereas a uncertainty-affine policy explores during training, but won't be safe in test. This work proposes an increasing penalty on model uncertainty to start explore, but converge uncertainty-averse. \XX{(NOTE: I am producing an according plot until Wednesday)}
% We train risk-affine, but still converge
% We account for uncertainty during training in a uncertainty-averse way and show that the training still converges to a policy.?
% Kahn is focused on velocity reduction and we are on regional avoidance?

\subsection{Collision avoidance with uncertainty estimates}

%We incorporate approximate uncertainty measures in a model-based reinforcement learning to avoid regions of unpredictable agents and drive more conservative during test. 

The RL framework is separated into a collision prediction and a minimal-cost action selection. On every step a neural network evaluates the action possibilities by predicting their future collision probability and its corresponding uncertainty. A model predictive controller (MPC) selects the safest action and executes it in the simulated environment. This process is repeated until an epoch ends in a collision or no collision. The action-history is labelled according to the collision result and used for a parameter update in the network. 

% Motion primitive generation
% Non-holonomic constraints or no constraints??
An LSTM network predicts each action's $u_{t:t+}$ collision probability $P\left(coll \vert s_{t-:t}, u_{t:t+}\right)$, given the car's and pedestrian's position history $s_{t-:t}$. The taken approaches distinguishes itself from supervised learning approach by the feedback loop on learning executed action histories. This allows the policy to predict collaborative actions from pedestrians with an understanding of its own future policy.

\textit{MC-Dropout} and \textit{Deep Ensembles} are used to get stochastic estimates of the model uncertainty. On each prediction we draw a sample mean and variance from multiple forward passes of each dropout-enriched network that is in the ensemble. 

A Model Predictive Control architecture selects the action with the minimal joint cost.
\begin{equation}
\begin{aligned}
& \hspace*{-.5in} u^\star_{t:t+n} = \argmin_{u\in U}\left(\lambda_v {\tt Var}(E[P_{\rm coll}]) + \right. \\
&\hspace*{.5in}  \left. \lambda_c P_{coll} + \lambda_g f_{\rm time\_to\_goal}\right)
\end{aligned}
\label{eq:min_cost} 
\end{equation}
The action is executed in simulation and the loop starts from the beginning.

Note that overly uncertainty-averse policies would not explore and find the optimal trajectory. Additionally,  the stochastic averaging during prediction reduces the ensembles diversity, which hinders explorative actions in early phases of training. To overcome this effect, the action selection process is noisified during early phases, similar as in $\epsilon-$greedy methods. Additionally, the penalty on highly uncertain actions is increased over time to remain explorative in early training phases, but finally act uncertainty-averse during execution. 

Another challenge is to design a simulator of pedestrian behavior. A \textit{gym} simulation environment \cite{Gym_2016} is implemented, that exhibits multiple agent behaviors that are following an ORCA, CADRL, non-cooperative or static policy. This way, the model will predict behaviors of similar pedestrians with low uncertainty and act conservative around pedestrians that behave different.


==> open_questions.tex <==
Discussion of plots

Answers:
Horizontal lines in uncertainty plots are caused by number of samples (i think)
The errors of a small model that overfits cannot be identified by uncertainty

Are the regions of uncertainty identifiable with regions of low probability? -- Do they correlate?

Point of Mike / My point:
- If I train risk-averse, can I ever learn?
- Can I act risk-averse, if I train risk-affine?

Point of Mike:
- How do other parameters (shape, velocity,...) influence the uncertainty?
- Where does the spatial uncertainty information come from? -- Why does my obst on the left not influence my prediction on the right?

When is new data new? (linked to - when is my model uncertain ?)
- In 1D, data is "newer", if the difference between its' value and the trained values is high.
  - The model, that has been overfitted on the training points, now shows a higher uncertainty the greater the distance of the new point is.
  - It highly depends on the model I am fittig
    - In 1D it looks like log-reg that is only uncertain at the decision boundary
    - How can it be uncertain outside of the decision boundaries, but at points with a high distance?
  - Jack's thesis:
    - Draws a uncertainty boundary for a 10dim space -- How can I draw this boundary -- My goal is to stay in it.
- How does this scale to 10D?
  - What is the "distance" metric, that causes models to exhibit different results
- This is probably well studied in Bayesian formulations?

Point of Shayegan:
- I need roll-out to learn how the current action is linked to the next action
  - In RL I assume to know what my agent will do in the next step
- During the roll-out RL offers convergence guarantees, while supervised learning, that is updated with environment feedback does (maybe?) not offer the guarantees!

Point of Nikita:
!Dropout is traditionally deactivated during execution to have a model that works. 
- Now if I sample and randomly deactivate nodes during test, I have other models and draw my model uncertainty from different models
- But with drawing an infinite number of samples, I approach the real model mean
- With this, I also approach the real model variance with infinite samples

Points of Arpan:
- Why is there two lines at 30deg, that have the same model uncertainty -- Show that other sample doesn't have these lines
- Why is do red points have low uncertainty and green points at intersection have high uncertainty?
 
Points of Jon:
- Make sure last plot shows, that I can develop safe policies with few data.
- Not only that uncertainty is explained away with more data

TODO:
Plot that drawing infinite samples lets the sample mean approach the mean.
!My approach can be applied to any existing NN collision avoidance!
Implement Bootstrapping!
